Service-oriented Context-aware Framework

Location- and context-aware services are emerging technologies in mobile and desktop environments, however, most of them are difficult to use and do not seem to be beneficial enough. Our research focuses on designing and creating a service-oriented framework that helps location- and context-aware, client-service type application development and use. Location information is combined with other contexts such as the users' history, preferences and disabilities. The framework also handles the spatial model of the environment (e.g. map of a room or a building) as a context. The framework is built on a semantic backend where the ontologies are represented using the OWL description language. The use of ontologies enables the framework to run inference tasks and to easily adapt to new context types. The framework contains a compatibility layer for positioning devices, which hides the technical differences of positioning technologies and enables the combination of location data of various sources.

==> eptcsdata.tex <==
\providecommand{\event}{M.H. ter Beek (Ed.): Young Researchers Workshop\\
on Service-Oriented Computing 2009 (YR-SOC'09).
}
\providecommand{\volume}{2}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{15}
\providecommand{\eid}{2}

